Quasi-Newton Methods for Saddle Point Problems and Beyond

This paper studies quasi-Newton methods for solving strongly-convex-strongly-concave saddle point problems (SPP). We propose greedy and random Broyden family updates for SPP, which have explicit local superlinear convergence rate of ${\mathcal O}\big(\big(1-\frac{1}{n\kappa^2}\big)^{k(k-1)/2}\big)$, where $n$ is dimensions of the problem, $\kappa$ is the condition number and $k$ is the number of iterations. The design and analysis of proposed algorithm are based on estimating the square of indefinite Hessian matrix, which is different from classical quasi-Newton methods in convex optimization. We also present two specific Broyden family algorithms with BFGS-type and SR1-type updates, which enjoy the faster local convergence rate of $\mathcal O\big(\big(1-\frac{1}{n}\big)^{k(k-1)/2}\big)$. Additionally, we extend our algorithms to solve general nonlinear equations and prove it enjoys the similar convergence rate.

==> experiment.tex <==
\section{Experiments}

\subsection{AUC Problem}
We consider the following AUC maximization problem which can be written in the form of:
\begin{eqnarray}
\label{eq:AUC}
\min_{\vx\in\BR^{n-1}}\max_{y\in\BR} f(\vx,y) \defeq \frac{1}{N} \sum_{i=1}^N f_i(\vx,y;\va_i,b_i,\lambda)
\end{eqnarray}
where $\vx=[\vw;u;v]^T$, and each component is defined as
\begin{align*}
    f_i(\vx,y;\va_i,b_i,\lambda) =\frac{\lambda}{2}\|\vx\|_2^2-p(1-p)y^2+(1-p)((\vw^T\va_i-u)^2-2(1+y)\vw^T\va_i)\mathbb{I}_{b_i=1}\\+p((\vw^T\va_i-v)^2+2(1+y)\vw^T\va_i)\mathbb{I}_{b_i=1}.
\end{align*}

\begin{eqnarray}
\hH_{\vw\vw}&=&\lambda \I +\frac{1}{N}\sum_i \left(2(1-p)\va_i\va_i^T\mathbb{I}_{b_i=1} +2p\va_i\va_i^T\mathbb{I}_{b_i=-1}\right)\\
\hH_{uu}&=&\lambda +\frac{1}{N}\sum_i 2(1-p)\mathbb{I}_{b_i=1}\\
\hH_{vv}&=&\lambda +\frac{1}{N}\sum_i 2p \mathbb{I}_{b_i=-1}\\
\hH_{\vw u}&=& -2(1-p)\frac{1}{N}\sum_i \va_i\mathbb{I}_{b_i=1}\\
\hH_{\vw v}&=& -2p\frac{1}{N}\sum_i \va_i\mathbb{I}_{b_i=-1}
\end{eqnarray}
Thus for a given direction $\h=(\h_\vw;\h_u;\h_v;\h_y)\in\RB^n$, Compute the Hessian-vector product:
\begin{eqnarray}
 \hH\h=\begin{bmatrix}
    \hH_{\vw\vw}\h_\vw+\hH_{\vw u} \h_u +\hH_{\vw v}\h_v+\hH_{\vw y}\h_y\\
    \hH_{\vw u}^{\top}\h_{\vw}+\hH_{uu}\h_u\\
    \hH_{\vw v}^{\top}\h_{\vw}+\hH_{vv}\h_v\\
    \hH_{\vw y}^{\top}\h_{\vw}+\hH_{yy}\h_{y}
    \end{bmatrix}.
\end{eqnarray}
where we can write $\hH_{\vw\vw}\h_{\w}$ as:
\begin{equation*}
   \hH_{\vw\vw}\h_{\vw} = \lambda \h_{\vw}+\frac{1}{N} \sum_{i} \left(2(1-p)\va_i^{\top}\h_{\vw} \va_i\mathbb{I}_{b_i=1} +2p \va_i^{\top}\h_{\vw}\va_i \mathbb{I}_{b_i-1}\right)
\end{equation*}

\section{Initialization}

Let $\mH = \hH^2\in\BR^{n\times n}$ and SVD of $\mH$ is $\H=\U{\bf \Lambda}\U^\top$. We want to find $\Q\in\BR^{d\times r}$ such that $\Q\approx\U$. We use the iteration
\begin{align*}
    \mQ_{k+1} =  {\rm orth}(\mH \mQ_{k}).
\end{align*}
After achieving $\mQ$, we estimate $\mH$ by
\begin{align*}
    \mH \approx (\mH \mQ) \mQ^\top + \alpha \mI.
\end{align*}
Since $\mH \mQ, \mQ\in\BR^{d\times r}$, the inverse of $\mH$ can be computed in $\fO(r^2 d)$.



==> random.tex <==
\section{Proof for Broyden Case}

\begin{proof}
Denote $\R\defeq \G-\H$, we
\begin{eqnarray}
\EB _{\u} \left[\frac{\u^{\top}\R \u}{\u^\top \H\u}\right]&\geq& \frac{1}{L^2}\EB \left[\frac{\u^{\top}\R\u}{\u^{\top}\u}\right]\\
&=&\frac{1}{L^2}{\rm tr}\left[\R\cdot \EB_{\u}\frac{\u\u^{\top}}{\u^{\top}\u}\right]\\
&=&\frac{1}{L^2n}{\rm tr}(\R) =\frac{1}{L^2 n} {\rm tr}(\R \cdot \I)\\
&\geq& \frac{\mu^2}{nL^2} {\rm tr} (\R \cdot \H^{-1}) =\frac{1}{n\kappa^2} \sigma_{\H}(\G)
\end{eqnarray}
Thus we have:
\begin{eqnarray}
\EB_{\u}[\sigma_{\H}(\G_{+})|\G] \leq \sigma_{\H}(\G) - \EB _{\u} \left[\frac{\u^{\top}\R \u}{\u^\top \H\u}\bigg|\G\right] \leq \left(1-\frac{1}{n\kappa^2}\right)\sigma_{\H}(\G)
\end{eqnarray}


\paragraph{Uniform spherical distribution:} Let $\vu\sim {\rm Unif}(\fS^{n-1})$, we have $\BE[\vu]=\vzero$ and $\Var(\vu)=\BE[\vu\vu^\top]=\frac{1}{n}\mI$. \url{https://stats.stackexchange.com/questions/22764/covariance-matrix-of-uniform-spherical-distribution} Hence,
\begin{align}
  &  \EB \left[\frac{\u^{\top}\R\u}{\u^{\top}\u}\right] \\
= &  \EB\left[{\rm tr}\left(\u^{\top}\R\u\right)\right] \\
= &  \EB\left[{\rm tr}\left(\R\u\u^{\top}\right)\right] \\
= &  {\rm tr}\left(\EB\left[\R\u\u^{\top}\right]\right) \\
= &  {\rm tr}\left(\R\EB\left[\u\u^{\top}\right]\right) \\
= &  {\rm tr}\left(\R\cdot\frac{1}{n}\I\right) \\
= &  \frac{1}{n}{\rm tr}\left(\R\right) 
\end{align}

\paragraph{Gaussian distribution:} Let $\vu\sim \fN_n(\vzero, \mI)$, then $\vu/\Norm{\vu}\sim {\rm Unif}(\fS^{n-1})$ (Exercise 3.3.7 of HDP book) which means
\begin{align*}
    \EB \left[\frac{\u\u^{\top}}{\u^{\top}\u}\right] = \frac{1}{n}\mI
\end{align*}
and
\begin{align}
  &  \EB \left[\frac{\u^{\top}\R\u}{\u^{\top}\u}\right] \\
=  &  \EB \left[{\rm tr}\left(\frac{\u^{\top}\R\u}{\u^{\top}\u}\right)\right] \\
=  &  {\rm tr}\left(\EB \left[\frac{\u^{\top}\R\u}{\u^{\top}\u}\right]\right) \\
=  &  {\rm tr}\left(\EB \left[\frac{\R\u\u^{\top}}{\u^{\top}\u}\right]\right) \\
=  &  {\rm tr}\left(\R\EB \left[\frac{\u\u^{\top}}{\u^{\top}\u}\right]\right) \\
=  &  {\rm tr}\left(\R\Cov\left[\vu/\norm{\vu}\right]\right) \\
=  &  \frac{1}{n}{\rm tr}\left(\R\right)
\end{align}

\end{proof}
